Doubt and Redundancy Kill Soft Errors -- Towards Detection and Correction of Silent Data Corruption in Task-based Numerical Software

Resilient algorithms in high-performance computing are subject to rigorous non-functional constraints. Resiliency must not increase the runtime, memory footprint or I/O demands too significantly. We propose a task-based soft error detection scheme that relies on error criteria per task outcome. They formalise how ``dubious'' an outcome is, i.e. how likely it contains an error. Our whole simulation is replicated once, forming two teams of MPI ranks that share their task results. Thus, ideally each team handles only around half of the workload. If a task yields large error criteria values, i.e.~is dubious, we compute the task redundantly and compare the outcomes. Whenever they disagree, the task result with a lower error likeliness is accepted. We obtain a self-healing, resilient algorithm which can compensate silent floating-point errors without a significant performance, I/O or memory footprint penalty. Case studies however suggest that a careful, domain-specific tailoring of the error criteria remains essential.

==> cartoons/control_flow_resilience_detection.tex <==
%\documentclass[tikz]{standalone}


\tikzstyle{decision} = [diamond, draw, fill=blue!20, 
    text width=2.5cm, minimum width=3cm, minimum height=1cm, text centered, node distance=2.5cm, inner sep=0pt, aspect=2]
\tikzstyle{block} = [rectangle, draw, fill=blue!20, 
    text width=5em, text centered, rounded corners, minimum height=4em]
\tikzstyle{line} = [draw, -latex']
\tikzstyle{cloudgreen} = [draw, ellipse,fill=green!20, node distance=3cm,
    minimum height=2em]
\tikzstyle{cloudred} = [draw, ellipse,fill=red!20, node distance=3cm,
    minimum height=2em]
\tikzstyle{cloudorange} = [draw, ellipse,fill=orange!20, node distance=3cm,
    minimum height=2em, text width=2.0cm]

\begin{figure}
\centering
\begin{tikzpicture}[node distance=2cm, auto]

\node [cloudgreen] (init) {start};
\node [decision, below of=init] (isDubious) {isDubious(res)};
\node [cloudgreen, right of=isDubious] (notdubious) {valid};
\node [decision, below left of=isDubious] (matches) {match($R$, $R'$)};
\node [cloudgreen, right of=matches,xshift=0.5cm] (match) {valid};
\node [cloudred, below left of=matches] (error) {soft error};

%\node [block, below left of=outcometriggered] (compute) {compute local outcome and set trigger};
%\node [decision, below of=compute] (checkRemote) {outcomes match};
%\node [cloudgreen, below left of=checkRemote] (completed) {set completed};
%\node [cloudred, below right of=checkRemote] (error) {trigger error};

%\node [block, below right of=outcometriggered] (copy) {copy outcome};
%\node [cloudgreen, below of=copy] (completed2) {set completed};

%\node [block, below right of=outcomeavailable,xshift=2cm] (compute2) {compute local outcome and set trigger};
%\node [decision, below of=compute2] (triggerCheck2) {local outcome triggered};
%\node [cloudorange, below left of=triggerCheck2,yshift=-1cm] (reschedule) {reschedule for check later};
%\node [block, below right of=triggerCheck2,yshift=-1cm] (share) {share outcome};
%\node [cloudgreen, below of=share] (completed3) {set completed};

\path [line] (init) -- (isDubious);
\path [line] (isDubious) -- node{no} (notdubious);
\path [line] (isDubious) -| node{yes} (matches);
\path [line] (matches) -- node{yes} (match);
\path [line] (matches) -| node{no} (error);

%yes for available
%\path [line] (outcomeavailable) -| node{yes} (outcometriggered);
%\path [line] (outcometriggered) -| node{yes} (compute);
%\path [line] (outcometriggered) -| node{no} (copy);
%\path [line] (copy) -- (completed2);
%\path [line] (compute) -- (checkRemote);
  %check remote
%\path [line] (checkRemote) -| node{yes}  (completed);
%\path [line] (checkRemote) -| node{no}  (error);

%no for available
%\path [line] (outcomeavailable) -| node{no} (compute2);
%\path [line] (compute2) -- (triggerCheck2);
%\path [line] (triggerCheck2) -| node{yes} (reschedule);
%\path [line] (triggerCheck2) -| node{no} (share);
%\path [line] (share) -- (completed3);

\end{tikzpicture}
\caption{Two-stage soft error detection process using redundancy and dubiosity checks. We assume to have an intermediate result $R$ that is to be checked against a redundantly computed result $R'$. $R$ and $R'$ should match if there is no corruption.}
\label{fig:checks}
\end{figure}
